Enabling Virtual Memory Research on RISC-V with a Configurable TLB Hierarchy for the Rocket Chip Generator

The Rocket Chip Generator uses a collection of parameterized processor components to produce RISC-V-based SoCs. It is a powerful tool that can produce a wide variety of processor designs ranging from tiny embedded processors to complex multi-core systems. In this paper we extend the features of the Memory Management Unit of the Rocket Chip Generator and specifically the TLB hierarchy. TLBs are essential in terms of performance because they mitigate the overhead of frequent Page Table Walks, but may harm the critical path of the processor due to their size and/or associativity. In the original Rocket Chip implementation the L1 Instruction/Data TLB is fully-associative and the shared L2 TLB is direct-mapped. We lift these restrictions and design and implement configurable, set-associative L1 and L2 TLB templates that can create any organization from direct-mapped to fully-associative to achieve the desired ratio of performance and resource utilization, especially for larger TLBs. We evaluate different TLB configurations and present performance, area, and frequency results of our design using benchmarks from the SPEC2006 suite on the Xilinx ZCU102 FPGA.

==> remarks.tex <==
\section{Final Remarks}
\label{sec:remarks}

We initially developed the configurable TLB Hierarchy on an older Rocket Chip commit \VK{mention which one commit/date} that supported the Xilinx ZCU102 platform. Unfortunately that repository does not track the recent changes in the Rocket Chip Generator. As a result, we opted to use the old Rocket Chip version for our evaluation with the Xilinx ZCU102 platform. In addition, to ensure the relevance and compatibility of our approach with more recent versions of Rocket Chip, we ported our design to the most recent version \VK{mention which commit/date} that also features new mechanisms such as a clustered L1 TLB \cite{pham} to further improve the TLB reach. We validated our ported design with simulations using Verilator, and we plan to evaluate it on other supported FPGA platforms.
\VK{I think that this information can be part of Section 4}

